From MIDI to Rich Tablatures: an Automatic Generative System incorporating Lead Guitarists' Fingering and Stylistic choices

Although the automatic identification of the optimal fingering for the performance of melodies on fretted string instruments has already been addressed (at least partially) in the literature, the specific case regarding lead electric guitar requires a dedicated approach. We propose a system that can generate, from simple MIDI melodies, tablatures enriched by fingerings, articulations, and expressive techniques. The basic fingering is derived by solving a constrained and multi-attribute optimization problem, which derives the best position of the fretting hand, not just the finger used at each moment.Then, by analyzing statistical data from the mySongBook corpus, the most common clich{\'e}s and biomechanical feasibility, articulations, and expressive techniques are introduced. Finally, the obtained output is converted into MusicXML format, which allows for easy visualization and use. The quality of the tablatures derived and the high configurability of the proposed approach can have several impacts, in particular in the fields of instrumental teaching, assisted composition and arranging, and computational expressive music performance models.

==> bends-fig.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=\columnwidth]{bends.pdf}
    \caption{Ratio of bent notes per string and amplitude in semitones (st).}
    \label{fig:bends}
\end{figure}


==> lick-1.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{lick-solution-1.png}
    \caption{Fingering generated by significantly penalizing position changes and finger spread and little penalizing string changes.}
    \label{fig:lick1}
\end{figure}


==> lick-2.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{lick-solution-2.png}
    \caption{Fingering generated by penalizing less position changes and finger spread and penalizing more string changes.}
    \label{fig:lick2}
\end{figure}


==> stats.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=\columnwidth]{playing-techniques.pdf}
    \caption{Ratio of notes in the corpus featuring expressive techniques for each string.
    Strings are labeled according to guitar standard tuning, the 6th string being the low E
    and the 1st string the high E.}
    \label{fig:techniques}
\end{figure}

